Missing Values Handling for Machine Learning Portfolios

We characterize the structure and origins of missingness for 159 cross-sectional return predictors and study missing value handling for portfolios constructed using machine learning. Simply imputing with cross-sectional means performs well compared to rigorous expectation-maximization methods. This stems from three facts about predictor data: (1) missingness occurs in large blocks organized by time, (2) cross-sectional correlations are small, and (3) missingness tends to occur in blocks organized by the underlying data source. As a result, observed data provide little information about missing data. Sophisticated imputations introduce estimation noise that can lead to underperformance if machine learning is not carefully applied.

==> exhibits/fcast-ew.tex <==
% latex table generated in R 4.1.3 by xtable 1.8-4 package
% Wed Nov  1 12:13:27 2023
   \multicolumn{5}{l}{\textit{Ad-hoc Imputations}} \\ 
Mean & 55 & \emph{55} &  & 51 & \emph{50} &  & 50 & \emph{50} &  & 31 & \emph{40} &  & 65 & \emph{66} &  & 66 & \emph{68} \\ 
  Ind / Size & 56 & \emph{56} &  & 53 & \emph{51} &  & 52 & \emph{50} &  & 43 & \emph{38} &  & 64 & \emph{64} &  & 65 & \emph{67} \\ 
  Last Obs & 56 & \emph{55} &  & 52 & \emph{49} &  & 52 & \emph{51} &  & 40 & \emph{37} &  & 65 & \emph{66} &  & 67 & \emph{68} \\ 
   \\ 
 \multicolumn{5}{l}{\textit{EM Imputations}} \\ 
EM & 58 & \emph{57} &  & 54 & \emph{52} &  & 55 & \emph{54} &  & 52 & \emph{51} &  & 65 & \emph{65} &  & 67 & \emph{68} \\ 
  EM AR1 & 56 & \emph{55} &  & 51 & \emph{49} &  & 53 & \emph{50} &  & 49 & \emph{48} &  & 64 & \emph{64} &  & 66 & \emph{67} \\ 
  pPCA10 & 57 & \emph{56} &  & 50 & \emph{49} &  & 54 & \emph{49} &  & 54 & \emph{53} &  & 65 & \emph{65} &  & 67 & \emph{68} \\ 


==> exhibits/fcast-vw.tex <==
% latex table generated in R 4.1.3 by xtable 1.8-4 package
% Wed Nov  1 12:13:27 2023
   \multicolumn{5}{l}{\textit{Ad-hoc Imputations}} \\ 
Mean & 31 & \emph{27} &  & 32 & \emph{21} &  & 27 & \emph{23} &  & 17 & \emph{25} &  & 40 & \emph{37} &  & 37 & \emph{40} \\ 
  Ind / Size & 31 & \emph{27} &  & 31 & \emph{21} &  & 28 & \emph{22} &  & 22 & \emph{12} &  & 37 & \emph{37} &  & 34 & \emph{40} \\ 
  Last Obs & 30 & \emph{26} &  & 38 & \emph{20} &  & 34 & \emph{21} &  & 23 & \emph{7} &  & 38 & \emph{38} &  & 35 & \emph{45} \\ 
   \\ 
 \multicolumn{5}{l}{\textit{EM Imputations}} \\ 
EM & 28 & \emph{19} &  & 36 & \emph{16} &  & 31 & \emph{18} &  & 32 & \emph{11} &  & 43 & \emph{34} &  & 39 & \emph{40} \\ 
  EM AR1 & 34 & \emph{21} &  & 35 & \emph{18} &  & 33 & \emph{18} &  & 27 & \emph{13} &  & 39 & \emph{33} &  & 36 & \emph{40} \\ 
  pPCA10 & 30 & \emph{23} &  & 34 & \emph{20} &  & 31 & \emph{18} &  & 32 & \emph{17} &  & 40 & \emph{33} &  & 38 & \emph{40} \\ 


==> exhibits/long_list.tex <==
% latex table generated in R 4.1.2 by xtable 1.8-4 package
% Sat Oct 21 08:26:17 2023
 streversal & Jegadeesh 1990 & 100.0 & 1 \\ 
  firmage & Barry and Brown 1984 & 100.0 & 2 \\ 
  indmom & Grinblatt and Moskowitz 1999 & 100.0 & 3 \\ 
  maxret & Bali, Cakici, and Whitelaw 2011 & 99.9 & 4 \\ 
  price & Blume and Husic 1973 & 99.8 & 5 \\ 
  size & Banz 1981 & 99.8 & 6 \\ 
  realizedvol & Ang et al. 2006 & 99.3 & 7 \\ 
  idiovol3f & Ang et al. 2006 & 99.2 & 8 \\ 
  high52 & George and Hwang 2004 & 99.1 & 9 \\ 
  returnskew3f & Bali, Engle and Murray 2015 & 99.0 & 10 \\ 
  zerotradealt1 & Liu 2006 & 98.7 & 11 \\ 
  dolvol & Brennan, Chordia, Subra 1998 & 97.8 & 12 \\ 
  returnskew & Bali, Engle and Murray 2015 & 96.6 & 13 \\ 
  idiovolaht & Ali, Hwang, and Trombley 2003 & 96.4 & 14 \\ 
  mom6m & Jegadeesh and Titman 1993 & 96.0 & 15 \\ 
  mom12moffseason & Heston and Sadka 2008 & 95.4 & 16 \\ 
  zerotrade & Liu 2006 & 94.9 & 17 \\ 
  volmkt & Haugen and Baker 1996 & 93.0 & 18 \\ 
  momseasonshort & Heston and Sadka 2008 & 91.9 & 19 \\ 
  mom12m & Jegadeesh and Titman 1993 & 91.6 & 20 \\ 
  coskewness & Harvey and Siddique 2000 & 91.2 & 21 \\ 
  pricedelayrsq & Hou and Moskowitz 2005 & 91.1 & 22 \\ 
  pricedelayslope & Hou and Moskowitz 2005 & 91.1 & 23 \\ 
  intmom & Novy-Marx 2012 & 91.0 & 24 \\ 
  coskewacx & Ang, Chen and Xing 2006 & 90.4 & 25 \\ 
  illiquidity & Amihud 2002 & 90.1 & 26 \\ 
  zerotradealt12 & Liu 2006 & 89.4 & 27 \\ 
  pricedelaytstat & Hou and Moskowitz 2005 & 88.3 & 28 \\ 
  mrreversal & De Bondt and Thaler 1985 & 85.0 & 29 \\ 
  shareiss1y & Pontiff and Woodgate 2008 & 84.9 & 30 \\ 
  herf & Hou and Robinson 2006 & 84.9 & 31 \\ 
  beta & Fama and MacBeth 1973 & 82.8 & 32 \\ 
  momseason & Heston and Sadka 2008 & 79.1 & 33 \\ 
  momoffseason & Heston and Sadka 2008 & 79.0 & 34 \\ 
  volsd & Chordia, Subra, Anshuman 2001 & 78.4 & 35 \\ 
  bookleverage & Fama and French 1992 & 76.8 & 36 \\ 
  roe & Haugen and Baker 1996 & 76.8 & 37 \\ 
  am & Fama and French 1992 & 76.7 & 38 \\ 
  cf & Lakonishok, Shleifer, Vishny 1994 & 76.7 & 39 \\ 
  hire & Bazdresch, Belo and Lin 2014 & 76.7 & 40 \\ 
  opleverage & Novy-Marx 2011 & 76.5 & 41 \\ 
  sp & Barbee, Mukherji and Raines 1996 & 76.4 & 42 \\ 
  leverage & Bhandari 1988 & 76.4 & 43 \\ 
  cashprod & Chandrashekar and Rao 2009 & 76.1 & 44 \\ 
  bpebm & Penman, Richardson and Tuna 2007 & 76.0 & 45 \\ 
  ebm & Penman, Richardson and Tuna 2007 & 76.0 & 46 \\ 
  numearnincrease & Loh and Warachka 2012 & 75.4 & 47 \\ 
  bm & Stattman 1980 & 74.4 & 48 \\ 
  roaq & Balakrishnan, Bartov and Faurel 2010 & 71.5 & 49 \\ 
  tax & Lev and Nissim 2004 & 69.7 & 50 \\ 
  gp & Novy-Marx 2013 & 68.4 & 51 \\ 
  betafp & Frazzini and Pedersen 2014 & 67.9 & 52 \\ 
  xfin & Bradshaw, Richardson, Sloan 2006 & 67.8 & 53 \\ 
  bidaskspread & Amihud and Mendelsohn 1986 & 67.7 & 54 \\ 
  betaliquidityps & Pastor and Stambaugh 2003 & 67.7 & 55 \\ 
  earnsupbig & Hou 2007 & 67.6 & 56 \\ 
  indretbig & Hou 2007 & 67.6 & 57 \\ 
  assetgrowth & Cooper, Gulen and Schill 2008 & 67.1 & 58 \\ 
  chinv & Thomas and Zhang 2002 & 67.1 & 59 \\ 
  delcoa & Richardson et al. 2005 & 67.1 & 60 \\ 
  dellti & Richardson et al. 2005 & 67.1 & 61 \\ 
  delequ & Richardson et al. 2005 & 67.1 & 62 \\ 
  dnoa & Hirshleifer, Hou, Teoh, Zhang 2004 & 67.1 & 63 \\ 
  lrreversal & De Bondt and Thaler 1985 & 67.0 & 64 \\ 
  grltnoa & Fairfield, Whisenant and Yohn 2003 & 66.9 & 65 \\ 
  totalaccruals & Richardson et al. 2005 & 66.8 & 66 \\ 
  noa & Hirshleifer et al. 2004 & 66.7 & 67 \\ 
  equityduration & Dechow, Sloan and Soliman 2004 & 66.7 & 68 \\ 
  accruals & Sloan 1996 & 66.6 & 69 \\ 
  chnwc & Soliman 2008 & 66.6 & 70 \\ 
  delcol & Richardson et al. 2005 & 66.6 & 71 \\ 
  chnncoa & Soliman 2008 & 66.5 & 72 \\ 
  delfinl & Richardson et al. 2005 & 66.5 & 73 \\ 
  delnetfin & Richardson et al. 2005 & 66.5 & 74 \\ 
  bmdec & Fama and French 1992 & 66.0 & 75 \\ 
  chinvia & Abarbanell and Bushee 1998 & 65.9 & 76 \\ 
  cheq & Lockwood and Prombutr 2010 & 65.6 & 77 \\ 
  cboperprof & Ball et al. 2016 & 65.3 & 78 \\ 
  chtax & Thomas and Zhang 2011 & 64.4 & 79 \\ 
  herfasset & Hou and Robinson 2006 & 64.2 & 80 \\ 
  herfbe & Hou and Robinson 2006 & 64.2 & 81 \\ 
  announcementreturn & Chan, Jegadeesh and Lakonishok 1996 & 64.1 & 82 \\ 
  rds & Landsman et al. 2011 & 63.6 & 83 \\ 
  investppeinv & Lyandres, Sun and Zhang 2008 & 62.9 & 84 \\ 
  netequityfinance & Bradshaw, Richardson, Sloan 2006 & 62.7 & 85 \\ 
  residualmomentum & Blitz, Huij and Martens 2011 & 62.2 & 86 \\ 
  pctacc & Hafzalla, Lundholm, Van Winkle 2011 & 62.0 & 87 \\ 
  abnormalaccruals & Xie 2001 & 62.0 & 88 \\ 
  entmult & Loughran and Wellman 2011 & 61.9 & 89 \\ 
  cfp & Desai, Rajgopal, Venkatachalam 2004 & 61.8 & 90 \\ 
  varcf & Haugen and Baker 1996 & 60.8 & 91 \\ 
  volumetrend & Haugen and Baker 1996 & 59.0 & 92 \\ 
  netdebtfinance & Bradshaw, Richardson, Sloan 2006 & 58.8 & 93 \\ 
  grcapx & Anderson and Garcia-Feijoo 2006 & 58.5 & 94 \\ 
  operprofrd & Ball et al. 2016 & 58.4 & 95 \\ 
  earningssurprise & Foster, Olsen and Shevlin 1984 & 58.4 & 96 \\ 
  ep & Basu 1977 & 57.6 & 97 \\ 
  grsaletogrinv & Abarbanell and Bushee 1998 & 57.4 & 98 \\ 
  grsaletogroverhead & Abarbanell and Bushee 1998 & 56.3 & 99 \\ 
  revenuesurprise & Jegadeesh and Livnat 2006 & 55.6 & 100 \\ 
  shareiss5y & Daniel and Titman 2006 & 55.6 & 101 \\ 
  chassetturnover & Soliman 2008 & 54.4 & 102 \\ 
  grcapx3y & Anderson and Garcia-Feijoo 2006 & 53.2 & 103 \\ 
  momseason06yrplus & Heston and Sadka 2008 & 52.7 & 104 \\ 
  momoffseason06yrplus & Heston and Sadka 2008 & 52.5 & 105 \\ 
  betatailrisk & Kelly and Jiang 2014 & 51.3 & 106 \\ 
  cash & Palazzo 2012 & 49.8 & 107 \\ 
  invgrowth & Belo and Lin 2012 & 47.2 & 108 \\ 
  feps & Cen, Wei, and Zhang 2006 & 46.8 & 109 \\ 
  analystrevision & Hawkins, Chamberlin, Daniel 1984 & 46.0 & 110 \\ 
  investment & Titman, Wei and Xie 2004 & 45.8 & 111 \\ 
  momseason11yrplus & Heston and Sadka 2008 & 45.3 & 112 \\ 
  momoffseason11yrplus & Heston and Sadka 2008 & 45.1 & 113 \\ 
  netpayoutyield & Boudoukh et al. 2007 & 43.9 & 114 \\ 
  intancfp & Daniel and Titman 2006 & 43.8 & 115 \\ 
  intanep & Daniel and Titman 2006 & 43.8 & 116 \\ 
  intansp & Daniel and Titman 2006 & 43.6 & 117 \\ 
  rev6 & Chan, Jegadeesh and Lakonishok 1996 & 43.6 & 118 \\ 
  std\_turn & Chordia, Subra, Anshuman 2001 & 43.2 & 119 \\ 
  intanbm & Daniel and Titman 2006 & 43.0 & 120 \\ 
  exclexp & Doyle, Lundholm and Soliman 2003 & 42.0 & 121 \\ 
  compositedebtissuance & Lyandres, Sun and Zhang 2008 & 41.7 & 122 \\ 
  compequiss & Daniel and Titman 2006 & 41.2 & 123 \\ 
  netdebtprice & Penman, Richardson and Tuna 2007 & 40.6 & 124 \\ 
  meanrankrevgrowth & Lakonishok, Shleifer, Vishny 1994 & 40.5 & 125 \\ 
  trendfactor & Han, Zhou, Zhu 2016 & 40.1 & 126 \\ 
  operprof & Fama and French 2006 & 38.1 & 127 \\ 
  payoutyield & Boudoukh et al. 2007 & 35.9 & 128 \\ 
  rd & Chan, Lakonishok and Sougiannis 2001 & 35.6 & 129 \\ 
  tang & Hahn and Lee 2009 & 34.9 & 130 \\ 
  frontier & Nguyen and Swanson 2009 & 33.6 & 131 \\ 
  fr & Franzoni and Marin 2006 & 33.0 & 132 \\ 
  adexp & Chan, Lakonishok and Sougiannis 2001 & 31.3 & 133 \\ 
  delbreadth & Chen, Hong and Stein 2002 & 30.0 & 134 \\ 
  forecastdispersion & Diether, Malloy and Scherbina 2002 & 29.3 & 135 \\ 
  earningsforecastdisparity & Da and Warachka 2011 & 28.3 & 136 \\ 
  earningsconsistency & Alwathainani 2009 & 27.3 & 137 \\ 
  realestate & Tuzel 2010 & 26.7 & 138 \\ 
  orgcap & Eisfeldt and Papanikolaou 2013 & 26.5 & 139 \\ 
  analystvalue & Frankel and Lee 1998 & 26.2 & 140 \\ 
  aop & Frankel and Lee 1998 & 26.2 & 141 \\ 
  fgr5yrlag & La Porta 1996 & 24.5 & 142 \\ 
  gradexp & Lou 2014 & 20.8 & 143 \\ 
  orderbacklog & Rajgopal, Shevlin, Venkatachalam 2003 & 20.2 & 144 \\ 
  shortinterest & Dechow et al. 2001 & 19.9 & 145 \\ 
  momseason16yrplus & Heston and Sadka 2008 & 19.8 & 146 \\ 
  orderbacklogchg & Baik and Ahn 2007 & 17.8 & 147 \\ 
  momoffseason16yrplus & Heston and Sadka 2008 & 16.6 & 148 \\ 
  predictedfe & Frankel and Lee 1998 & 14.8 & 149 \\ 
  ageipo & Ritter 1991 & 14.2 & 150 \\ 
  earningsstreak & Loh and Warachka 2012 & 14.1 & 151 \\ 
  ps & Piotroski 2000 & 14.1 & 152 \\ 
  sfe & Elgers, Lo and Pfeiffer 2001 & 11.6 & 153 \\ 
  rdcap & Li 2011 & 11.6 & 154 \\ 
  brandinvest & Belo, Lin and Vitorino 2014 & 11.0 & 155 \\ 
  retconglomerate & Cohen and Lou 2012 & 8.4 & 156 \\ 
  customermomentum & Cohen and Frazzini 2008 & 4.9 & 157 \\ 
  rdability & Cohen, Diether and Malloy 2013 & 2.3 & 158 \\ 
  io\_shortinterest & Asquith Pathak and Ritter 2005 & 0.2 & 159 \\ 
  

==> exhibits/one_signal_ew.tex <==
% latex table generated in R 4.1.3 by xtable 1.8-4 package
% Wed Nov  1 12:13:26 2023
   \multicolumn{7}{l}{Mean Return (\% Ann)} \\ & EM Imputed & -1.2 &  2.9 &  7.1 & 12.7 & 17.5 \\ 
   & Missing Dropped & -0.1 &  3.1 &  6.2 & 10.2 & 15.2 \\ 
   \cmidrule{2-7} & \emph{EM Improvement} & \emph{-2.0} & \emph{-0.3} & \emph{ 0.5} & \emph{ 2.1} & \emph{ 4.4} \\ 
   \\ \multicolumn{7}{l}{Sharpe Ratio (Ann)} \\ & EM Imputed & -0.05 &  0.16 &  0.58 &  0.86 &  1.21 \\ 
   & Missing Dropped & -0.01 &  0.26 &  0.53 &  0.89 &  1.11 \\ 
   \cmidrule{2-7} & \emph{EM Improvement} & \emph{-0.22} & \emph{-0.04} & \emph{ 0.01} & \emph{ 0.09} & \emph{ 0.18} \\ 


==> exhibits/one_signal_vw.tex <==
% latex table generated in R 4.1.3 by xtable 1.8-4 package
% Wed Nov  1 12:13:26 2023
   \multicolumn{7}{l}{Mean Return (\% Ann)} \\ & EM Imputed & -1.9 &  0.5 &  3.1 &  7.0 & 11.2 \\ 
   & Missing Dropped & -2.1 &  0.8 &  2.6 &  5.5 & 10.4 \\ 
   \cmidrule{2-7} & \emph{EM Improvement} & \emph{-1.5} & \emph{-0.4} & \emph{ 0.2} & \emph{ 1.5} & \emph{ 3.8} \\ 
   \\ \multicolumn{7}{l}{Sharpe Ratio (Ann)} \\ & EM Imputed & -0.13 &  0.04 &  0.22 &  0.43 &  0.54 \\ 
   & Missing Dropped & -0.12 &  0.04 &  0.22 &  0.36 &  0.51 \\ 
   \cmidrule{2-7} & \emph{EM Improvement} & \emph{-0.10} & \emph{-0.04} & \emph{ 0.00} & \emph{ 0.06} & \emph{ 0.19} \\ 


==> exhibits/pct_obs_by_nsignal.tex <==
% latex table generated in R 4.1.3 by xtable 1.8-4 package
% Wed Nov  1 12:13:26 2023
  25 &  & 89.2 & 49.7 &  & 96.2 & 86.4 &  & 95.8 & 88.1 \\ 
  50 &  & 82.1 & 37.4 &  & 87.9 & 42.1 &  & 91.0 & 53.5 \\ 
  75 &  & 76.2 & 9.7 &  & 81.3 & 16.1 &  & 85.7 & 23.8 \\ 
  100 &  & 71.3 & 0.0 &  & 76.7 & 10.1 &  & 81.4 & 11.2 \\ 
  125 &  & 63.2 & 0.0 &  & 70.7 & 0.9 &  & 75.0 & 0.8 \\ 
  150 &  & 55.8 & 0.0 &  & 63.5 & 0.0 &  & 67.6 & 0.0 \\ 


==> exhibits/pct_obs_one_signal_ptile.tex <==
% latex table generated in R 4.1.3 by xtable 1.8-4 package
% Wed Nov  1 12:13:25 2023
  5 &  & 0 & 0 & 3 & 14 & 14 & 15 & 16 \\ 
  25 &  & 25 & 34 & 42 & 43 & 45 & 45 & 50 \\ 
  50 &  & 67 & 53 & 66 & 66 & 69 & 71 & 74 \\ 
  75 &  & 82 & 72 & 80 & 78 & 79 & 87 & 89 \\ 
  95 &  & 100 & 97 & 97 & 99 & 99 & 99 & 99 \\ 


==> exhibits/temp.tex <==
% latex table generated in R 4.2.3 by xtable 1.8-4 package
% Mon Oct 16 15:03:35 2023
\begin{tabular}{rrrrrrrrr}
   5 &  & 0.0 & 0.0 & 3.3 & 13.9 & 13.3 & 14.7 & 15.6 \\ 
  25 &  & 21.8 & 34.4 & 41.8 & 42.8 & 43.3 & 44.7 & 50.0 \\ 
  50 &  & 66.8 & 52.4 & 66.4 & 65.5 & 68.9 & 70.3 & 74.0 \\ 
  75 &  & 82.4 & 71.5 & 79.7 & 77.8 & 79.1 & 86.9 & 88.8 \\ 
  95 &  & 99.6 & 96.9 & 97.4 & 99.1 & 99.3 & 99.0 & 99.3 \\ 
  \end{tabular}

